Geometric analysis of Oscillations in the Frzilator model

A biochemical oscillator model, describing developmental stage of myxobacteria, is analyzed mathematically. Observations from numerical simulations show that in a certain range of parameters, the corresponding system of ordinary differential equations displays stable and robust oscillations. In this work, we use geometric singular perturbation theory and blow-up method to prove the existence of a strongly attracting limit cycle. This cycle corresponds to a relaxation oscillation of an auxiliary system, whose singular perturbation nature originates from the small Michaelis-Menten constants of the biochemical model. In addition, we give a detailed description of the structure of the limit cycle, and the timescales along it.

==> subfiles/AppRedProb.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Analysis of \hjk{\S_{0,4}} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{lemma}[\textcolor{red}{checked!}] 
%The critical manifold $\hjk{\S_{0,4}}$ has the following properties. 
%\begin{enumerate}
%\item 
% For sufficiently small $\delta>0$, there exist $\ve_0>0$ and a smooth function $\hjk{h_{\ve,4}}(c,e)$ defined on $\hjk{I_4^\txta}=\left[\delta,\ 1-\delta\right]\times\left[\delta, \ \gamma - \delta\right]$ such that the manifold 
% \begin{equation}
% \hjk{\S_{0,4}}_{a,\ve}=\left\{ (f,c,e)\in\C\, | \, f=1+\hjk{h_{\ve,4}}(c,e), \, (c,e)\in \hjk{I_4^\txta} \right\},
% \end{equation}
% is a locally invariant attracting manifold of $X_\ve$ for $\ve\in(0,\ve_0]$. The function $\hjk{h_{\ve,4}}(c,e)$ has the expansion
% \begin{equation}
% \hjk{h_{\ve,4}}(c,e) = \frac{e}{e - \gamma}\ve + O(\ve^2)
% \end{equation}

%\item 
% The slow flow along $\hjk{\S_{0,4}}_a$, defined as $X^4_a=\lim_{\ve\to 0}\frac{1}{\ve}X_\ve|_{\hjk{\S_{0,4}}_a}$ is given as
% \begin{equation}\label{Red4_a}
% \begin{split}
% \dot c & = -\frac{64 \gamma ce(c-1)(e-1)}{e-\gamma}\\
% \dot e & =  \frac{64 \gamma ce(c-1)(e-1)(1-2c)}{e-\gamma}
% \end{split}
% \end{equation}
% The phase portrait of \eqref{Red4_a} is shown in Figure \ref{fS4}.

% % \begin{figure}\centering
% % \includegraphics[]{figures/redVF4}
% % \caption{Flow of the slow vector field on $\hjk{\S_{0,4}}$.}
% % \label{fS4}
% % \end{figure}

%\end{enumerate}
%\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Analysis of \hjk{\S_{0,5}} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{lemma} [\textcolor{red}{checked!}]
%The critical manifold $\hjk{\S_{0,5}}$ has the following properties.
%\begin{enumerate}
%\item 
% For sufficiently small $\delta>0$, there exist $\ve_0>0$ and a smooth function $\hjk{h_{\ve,5}}(f,e)$ defined on $\hjk{I_5^\txta}=\left[\frac{1}{2}+\delta,\ 1-\delta\right]\times\left[\delta,\ 1-\delta\right]$ such that the manifold 
% \begin{equation}
% \hjk{\S_{0,5}}_{a,\ve}=\left\{ (f,c,e)\in\C\, | \, c=\hjk{h_{\ve,5}}(f,e), \, (f,e)\in \hjk{I_5^\txta} \right\},
% \end{equation}
% is a locally invariant attracting manifold of $X_\ve$ for $\ve\in(0,\ve_0]$. The function $\hjk{h_{\ve,5}}(f,e)$ has the expansion
% \begin{equation}
% \hjk{h_{\ve,5}}(f,e) = 1+\frac{1}{2(1-2f)}\ve + O(\ve^2)
% \end{equation}

%\item 
%The slow flow along $\hjk{\S_{0,5}}_a$, defined as $X^5_a=\lim_{\ve\to0}\frac{1}{\ve}X_\ve|_{\hjk{\S_{0,5}}_a}$ is given as
% \begin{equation}\label{Red5_a}
% \begin{split}
% \dot f &= \frac{32 e f^2(e-1)(f-1)(\gamma - e)}{2f-1}\\
% \dot e &=\frac{64 e f^2(e-1)(f-1)}{2f-1}
% \end{split}
% \end{equation}
% The phase portrait of \eqref{Red5_a} is shown in Figure \ref{fS5}.

% % \begin{figure}\centering
% % \includegraphics[]{figures/redVF5}
% % \caption{Flow of the slow vector field on $\hjk{\S_{0,5}}$.}
% % \label{fS5}
% % \end{figure}

%\end{enumerate}
%\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Analysis of S^6 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{lemma} [\textcolor{red}{checked!}]
%The critical manifold $S^6$ has the following properties.
%\begin{enumerate}
%\item 
% For sufficiently small $\delta>0$, there exist $\ve_0>0$ and a smooth function $h^6_\ve(f,c)$ defined on $I^6_a=\left[\frac{1}{2}+\delta,1-\delta\right]\times\left[\delta,1-\delta\right]$ such that the manifold 
% \begin{equation}
% S^6_{a,\ve}=\left\{ (f,c,e)\in\C\, | \, e=\hjk{h_{\ve,5}}(f,c), \, (f,c)\in I_a^6 \right\},
% \end{equation}%
% is a locally invariant attracting manifold of $X_\ve$ for $\ve\in(0,\ve_0]$. 
% The function $h^6_\ve$ has the expansion
% \begin{equation}
% h^6_\ve(f,c) = 1 + \frac{1}{2(1-2c)}\ve + O(\ve^2)
% \end{equation}

%\item 
% The slow flow along $S^6_a$, defined as $X^6_a=\lim_{\ve\to0}\frac{1}{\ve}X_\ve|_{S^6_a}$ is given as
% \begin{equation}\label{Red6_a}
% \begin{split}
% \dot f &= \frac{32(\gamma-1)fc^2(c-1)(f-1)}{2c-1}\\
% \dot c &=  \frac{64c^2f(c-1)(f-1)(2f-1)}{2c-1}
% \end{split}
% \end{equation}
% The phase portrait of \eqref{Red6_a} is shown in Figure \ref{fS6}.

% % \begin{figure}\centering
% % \includegraphics[]{figures/redVF6}
% % \caption{Flow of the slow vector field on $S^6$.}
% % \label{fS6}
% % \end{figure}
%\end{enumerate}
%\end{lemma}
%%%%%%%%%%%%%%%%%%% THESE ARE CORRECT, BUT WE SKIP THEM %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% THESE ARE CORRECT, BUT WE SKIP THEM %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% THESE ARE CORRECT, BUT WE SKIP THEM %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% THESE ARE CORRECT, BUT WE SKIP THEM %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% THESE ARE CORRECT, BUT WE SKIP THEM %%%%%%%%%%%%%%%
{\color{pink}
\begin{lemma}\label{App.h}
The critical manifolds $\hjk{\S_{0,4}}$ and $\hjk{\S_{0,5}}$ have the following properties:
\begin{enumerate}
\item For sufficiently small $\delta>0$, there exist $\ve_0>0$ and a smooth function $\hjk{h_{\ve,4}}(c,e)$ defined on $\hjk{I_4^\txta}=\left[\delta,\ 1-\delta\right]\times\left[\delta, \ \gamma - \delta\right]$ such that the manifold 
\begin{equation}
\hjk{\S_{\ve,4}^\txta}=\left\{ (f,c,e)\in\C\, | \, f=1+\hjk{h_{\ve,4}}(c,e), \, (c,e)\in \hjk{I_4^\txta} \right\},
\end{equation}
is a locally invariant attracting manifold of $X_\ve$ for $\ve\in(0,\ve_0]$. The function $\hjk{h_{\ve,4}}(c,e)$ has the expansion
\begin{equation}
\hjk{h_{\ve,4}}(c,e) = \frac{e}{e - \gamma}\ve + O(\ve^2)
\end{equation}
%%%%%%-------------------------------
\item For sufficiently small $\delta>0$, there exist $\ve_0>0$ and a smooth function $\hjk{h_{\ve,5}}(f,e)$ defined on $\hjk{I_5^\txta}=\left[\frac{1}{2}+\delta,\ 1-\delta\right]\times\left[\delta,\ 1-\delta\right]$ such that the manifold 
\begin{equation}
\hjk{\S_{\ve,5}^\txta}=\left\{ (f,c,e)\in\C\, | \, c=\hjk{h_{\ve,5}}(f,e), \, (f,e)\in \hjk{I_5^\txta} \right\},
\end{equation}
is a locally invariant attracting manifold of $X_\ve$ for $\ve\in(0,\ve_0]$. The function $\hjk{h_{\ve,5}}(f,e)$ has the expansion
\begin{equation}
\hjk{h_{\ve,5}}(f,e) = 1+\frac{1}{2(1-2f)}\ve + O(\ve^2)
\end{equation}
%%%%%%%%-----------------------------
\end{enumerate}
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{App.SlowFlow}
The slow flows on $\hjk{\S_{0,4}}$ and $\hjk{\S_{0,5}}$ are given as follows:
\begin{enumerate}
\item The slow flow along $\hjk{\S_{0,4}^\txta}$, defined as $X^4_a=\lim_{\ve\to 0}\frac{1}{\ve}X_\ve|_{\hjk{\S_{\ve,4}^\txta}}$ is given as
\begin{equation}\label{Red4_a}
\begin{split}
\dot c & = \frac{-64 \gamma ce(c-1)(e-1)}{e-\gamma}\\
\dot e & =  \frac{64 \gamma ce(c-1)(e-1)(1-2c)}{e-\gamma}
\end{split}
\end{equation}
The phase portrait of \eqref{Red4_a} is shown in Figure \ref{fS4}.
\begin{figure}[H]
\centering
\includegraphics[]{figures/redVF4}
\caption{Flow of the slow vector field on $\hjk{\S_{0,4}}$.}
\label{fS4}
\end{figure}
%%%%%%%------------------------------------
\item The slow flow along $\hjk{\S_{0,5}^\txta}$, defined as $X^5_a=\lim_{\ve\to0}\frac{1}{\ve}X_\ve|_{\hjk{\S_{\ve,5}^\txta}}$ is given as
\begin{equation}\label{Red5_a}
\begin{split}
\dot f &= \frac{32 e f^2(e-1)(f-1)(\gamma - e)}{2f-1}\\
\dot e &=\frac{64 e f^2(e-1)(f-1)}{2f-1}
\end{split}
\end{equation}
The phase portrait of \eqref{Red5_a} is shown in Figure \ref{fS5}.
\begin{figure}[H]
\centering
\includegraphics[]{figures/redVF5}
\caption{Flow of the slow vector field on $\hjk{\S_{0,5}}$.}
\label{fS5}
\end{figure}
%%%%%%%%%%%%%%-------------------------------
\end{enumerate}
\end{lemma}
}

==> subfiles/GlobalUniqueness.tex <==
% In this subsection we show that for sufficiently small $\ve>0$, almost all solutions of system~\eqref{repara}, and equivalently system~\eqref{syseps}, converge to a ``unique'' limit cycle.
% As mentioned in Subsection~\ref{critical.manifold}, away from the critical manifold $S$, the linear system~\eqref{identical} is identical to the layer problem~\eqref{layer}.
% The eigenvalues of system~\eqref{identical} are given by $\lambda_1=-2\alpha$ and $\lambda_{2,3}=\alpha\pm i\beta$, for some $\alpha, \beta>0$.
% In fact, the layer problem has a one-dimensional stable manifold and a two-dimensional unstable manifold.
% As the layer problem~\eqref{identical} is a linear system, we can explicitly calculate the closed form of the solutions.
% It is verified that, by solving system~\eqref{identical}, the components $f(t)$, $c(t)$ and $e(t)$ can be written in the form 
% \begin{equation}\label{sol.layer}
% \rho_1+\rho_2e^{-2\alpha t}+\rho_3\sin(\beta t) e^{\alpha t}+\rho_4\cos(\beta t) e^{\alpha t},
% \end{equation}
% for some $\rho_j\in\mathbb{R}$, $j=1,2,3,4$.
% Equation~\eqref{sol.layer} clearly shows that if the layer problem is started from the interior of the cube $\C$, it will reach one of the attracting manifolds $S_a^j$ $(j=1,2,...,6)$ in a \emph{finite time}.
% %Moreover, in \cite{taghvafard2017parameter} it is proven that the cube $\C$ is forward invariant, i.e., 
% Therefore, it remains to show that a trajectory, starting from any point in $S_a^j$, will converge to the singular cycle, depicted in Fig.~\ref{SinCyc}.



% {\color{red}{[@Hadi: I suggest you make a comment about uniqueness up to exponential closedness. Recall that the manifolds from Fenichel are in general not unique, but since they are exponentially close, any of them is called the slow-manifold. This is translated to the fact that in this case uniqueness is by identifying all exponentially closed manifolds. Maybe this is what you meant by "unique" (between "") but need a clarification. ]}}






























% \newpage

==> subfiles/Outline.tex <==
To be written ...
